About evaluation metrics for contextual uplift modeling

In this tech report we discuss the evaluation problem of contextual uplift modeling from the causal inference point of view. More particularly, we instantiate the individual treatment effect (ITE) estimation, and its evaluation counterpart. First, we unify two well studied fields: the statistical ITE approach and its observational counterpart based on uplift study. Then we exhibit the problem of evaluation, based on previous work about ITE and uplift modeling. Moreover, we derive a new estimator for the uplift curve, built on logged bandit feedback dataset, that reduces its variance. We prove that AUUC fails on non randomized control trial (RCT) datasets and discuss some corrections and guidelines that should be kept in mind while using AUUC (re-balancing the population, local importance sampling using propensity score).

==> PomonaLgcsFormatting.tex <==
%%% This file is the preamble for the Pomona Linguistics LaTeX Paper Template, which is also used for the Quick Reference Guide. If you are brand new to writing with LaTeX, we suggest NOT messing with it, and just writing your paper using the Paper Template. If you are getting more comfortable in LaTeX and want to add packages and commands, this is where you do it (when using this template).

%For stacking text, used here in autosegmental diagrams
\usepackage{stackengine}

%To combine rows in tables
\usepackage{multirow}

%geometry helps manage margins, among other things.
\usepackage[margin=1in]{geometry}

%Gives some extra formatting options, e.g. underlining/strikeout
\usepackage{ulem}

%For putting links into papers, also helps make cross-references in the paper smart references
\usepackage[colorlinks = true,
            linkcolor = blue,
            urlcolor  = blue,
            citecolor = blue,
            anchorcolor = blue]{hyperref} %smarter cross-references, these options turn links blue

%Use package/command below to create a double-spaced document, if you want one. Uncomment BOTH the package and the command (\doublespacing) to create a doublespaced document, or leave them as is to have a single-spaced document.
%\usepackage{setspace}
%\doublespacing 

%paragraph formatting
\usepackage[parfill]{parskip}
\setlength{\parskip}{5pt} %plus 1 minus 1}
\setlength{\parindent}{30pt}
\usepackage{titlesec}

%use for special OT tableaux symbols like bomb and sad face. must be loaded early on because it doesn't play well with some other packages
\usepackage{fourier-orns}

%Basic math symbols 
\usepackage{pifont}
\usepackage{amssymb}

%%%Gives shortcuts for glossing. The use of this package is NOT explained in the Quick Reference Guide, but the documentation is on CTAN for those that are interested. MJKD finds it handy for glossing. (https://ctan.org/pkg/leipzig?lang=en)
\usepackage{leipzig}

%Tables
\usepackage{caption} %For table captions
\usepackage{booktabs} %helps format tables

%For citations and bibliography - as of 9.1.2019 we don't explain citations in this Quick Reference Guide, but Pedro Martin's tutorial does (see links in the Guide).
\usepackage{natbib}

%For OT-style tableaux
\usepackage{ot-tableau}

%Fonts
%\usepackage[no-math]{fontspec} %This allows you to enter (via an IPA kayboard) IPA fonts and other symbols directly into LaTeX. Requires a particular setyp, see below.
\usepackage{libertine} %A font that actually contains many IPA symbols. This is the font you see in the preview to the right.

%to use these fonts, be sure that your typesetting engine is set to "XeLaTeX." In Overleaf, go to the Menu link on the top left (by the Overleaf icon), and under Settings be sure that the Compiler is set to "XeLaTeX." If you accessed this document via the Overleaf Pomona Linguistics template, all of this was already done for you.

%The Pomona Linguistics Paper Template in Overleaf is already set up for this, but you may run into this problem if you start building your own documents.

%highlights text with \hl{text}
\usepackage{color, soul}

%Drawing Syntax Trees
\usepackage[linguistics]{forest}

%This specifies some formatting for the forest trees to make them nicer to look at
\forestset{
  nice nodes/.style={
    for tree={
      inner sep=0pt,
      fit=band,
    },
  },
  default preamble=nice nodes,
}

%% For numbered and glossed examples %%
\usepackage{gb4e}



%Changes the \maketitle command to be smaller and take up less space on a page. 
\makeatletter         
\def\@maketitle{   % custom maketitle 
\noindent {\Large \bfseries \color{black} \@title}  \\ \hrule \noindent \@author \\ \@date  
}

%The code below will draw a circle around a piece of text. This is very useful for drawing attention to a word in a data example. use the command \circled{text} where the argument (`text' here) is what you want to be circled. This is illustrated in the Quick Reference Guide and the Paper Template.

\usepackage{tikz}

\newcommand{\circled}[1]{\begin{tikzpicture}[baseline=(word.base)]
\node[draw, rounded corners, text height=8pt, text depth=2pt, inner sep=2pt, outer sep=0pt, use as bounding box] (word) {#1};
\end{tikzpicture}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Useful Ling Shortcuts

\RequirePackage{leipzig}
%\RequirePackage{mathtools} % for \mathrlap

% % % Shortcuts  (borrowed from JZ, I'm still unsure exactly what xspace requires)
\RequirePackage{xspace}
\xspaceaddexceptions{]\}}

%This makes the \emptyset command be a nicer one
\let\oldemptyset\emptyset
\let\emptyset\varnothing
\newcommand{\nothing}{$\emptyset$}

%Not all of these are explained in the Quick Reference Guide, but they are here bc they are relevant to some of our students.
\newcommand{\1}{\rlap{$'$}\xspace}
\newcommand{\0}{\rlap{\textsuperscript{$ˆ{\circ}$}}\xspace}
\newcommand{\Lb}[1]{$\text{[}_{\text{#1}}$ } %A more convenient left bracket
\newcommand{\Rb}[1]{$\text{]}_{\text{#1}}$ } %A more convenient left bracket
\newcommand{\gap}{\underline{\hspace{1.2em}}}
\newcommand{\vP}{\emph{v}P}
\newcommand{\lilv}{\emph{v}}
\newcommand{\Abar}{A$'$-} %A more convenient A-bar notation
\newcommand{\ph}{$\varphi$\xspace} %A more convenient phi
\newcommand{\pro}{\emph{pro}\xspace}
\newcommand{\subs}[1]{\textsubscript{#1}} %A more convenient subscript
%\newcommand{\hd}{$^{\circ}$\xspace} %Symbol for printing head / degree symbol
\newcommand{\spells}{$\Longleftrightarrow$} %spellout arrow for morph spellout rules
\newcommand{\tr}[1]{\textit{t}\textsubscript{\textit{#1}}} %easy traces with subscript
\newcommand{\supers}[1]{\textsuperscript{#1}}

% Abbreviations for glossing, based on Leipzig
\newleipzig{hab}{hab}{habitual}
\newleipzig{rem}{rem}{remote}
\newleipzig{sm}{sm}{subject marker}
\newleipzig{t}{t}{tense}
\newleipzig{aa}{aa}{anti-agreement}
\newleipzig{pron}{pron}{pronoun}
\newleipzig{rec}{rec}{recent}
\newleipzig{om}{om}{object marker}
%\newleipzig{ipfv}{ipfv}{imperfective}
\newleipzig{asp}{asp}{aspect}
\newleipzig{lk}{lk}{linker}
\newleipzig{pcl}{pcl}{particle}
\newleipzig{stat}{stat}{stative}
\newleipzig{ints}{ints}{intensive}
\newleipzig{ascl}{ascl}{assertive subject clitic}
\newleipzig{nascl}{nascl}{non-assertive subject clitic}
\newleipzig{ta}{ta}{tense and/or aspect}
\newleipzig{assoc}{assoc}{associative marker}
\newleipzig{hon}{hon}{honorific}
%\newleipzig{whprt}{wh}{\wh particle}
\newleipzig{sa}{sa}{subject agreement}
\newleipzig{conj}{conj}{conjunction}
%\newleipzig{loc}{loc}{locative}
\newleipzig{expl}{expl}{expletive}
\newleipzig{rcm}{rcm}{reciprocal marker}
\newleipzig{pers}{pers}{persistive}
%\newleipzig{}{}{} %this is just to copy for when I want to add more

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%A couple of packages that seemed to prefer being called toward the end of the preamble

%This package provides macros for typesetting SPE-style phonological rules.
\usepackage{phonrule}

%For using Greek letters outside of math mode.
\usepackage{textgreek}


%Random, lets us use the XeLaTeX logo. Not important to the template at all.
\usepackage{metalogo}


%%%%%%%%%%%%
%% This is the end of the PREAMBLE
%%%%%%%%%%%

